Momentum mappings for subtractions at higher orders in QCD

Subtraction schemes provide a systematic way to compute fully-differential cross sections beyond the leading order in the strong coupling constant. These methods make singular real-emission corrections integrable in phase space by the addition of suitable counterterms. Such counterterms may be defined using momentum mappings, which are parametrisations of the phase space that factorise the variables that describe the particles becoming unresolved in some infrared or collinear limit from the variables that describe an on-shell phase space for the resolved particles. In this work, we review existing momentum mappings in a unified framework and introduce new ones for final-collinear and soft counterterms. The new mappings work in the presence of massive particles and with an arbitrary number of soft particles or of clusters of collinear particles, making them fit for subtraction methods at any order in perturbation theory. The new mapping for final-collinear counterterms is also used to elucidate relations among existing final-collinear mappings.

==> initialcoll.tex <==
\section{Two-sided initial-collinear mapping}
\label{sec:initial}


Since most initial-collinear momentum mappings were developed
for subtractions at \gls{NLO},
a kinematic configuration that generates a collinear divergence
but is poorly studied from the point of view of momentum mappings
takes place in hadron-hadron collisions
when the particles $\set{m+1, \ldots, m+k_a}$ in the final state
are collinear to the initial-state parton $a$
and the particles $\set{m+k_a+1, \ldots, m+k_a+k_b}$ in the final-state
are collinear to the other parton $b$.
Let
\begin{equation}
	p_A^\mu = p_a^\mu - \sum_{i=m+1}^{m+k_a} p_i^\mu,
	\qquad
	p_B^\mu = p_b^\mu - \sum_{j=m+k_a+1}^{m+k_a+k_b} p_j^\mu,
\end{equation}
and define
\begin{equation}
	x_a = \sqrt{
		\frac{(p_A+p_B)^2}{(p_a+p_B)^2}
		\frac{(p_A+p_b)^2}{(p_a+p_b)^2}
	},
	\qquad
	x_b = \sqrt{
		\frac{(p_A+p_B)^2}{(p_A+p_b)^2}
		\frac{(p_a+p_B)^2}{(p_a+p_b)^2}
	}.
\end{equation}
A valid momentum mapping is
\begin{equation}
	\tilde{p}_a^\mu = x_a p_a^\mu,
	\qquad
	\tilde{p}_b^\mu = x_b p_b^\mu,
	\qquad
	\tilde{p}_r^\mu =
	\Lambda[x_a p_a + x_b p_b, p_A + p_B]^\mu{}_\nu p_r^\nu
	\quad 1 \le r \le m.
\end{equation}

Note that in the limit of one of the bunches of final-state particles
being exactly collinear to the respective incoming parton,
\begin{equation}
	p_j^\mu = x_j p_b^\mu \quad m+k_a+1 \le m+k_a+k_b,
\end{equation}
we have
\begin{equation}
	p_B^\mu = \brk*{1- \sum_{j=m+k_a+1}^{m+k_a+k_b} x_j} p_b^\mu
	\equiv x_B p_b^\mu.
\end{equation}
This gives 

% Conserve the invariant mass of recoilers
For $2 \to 1$ processes like inclusive Higgs or vector boson production
there may be a single resolved particle in the final state.
A momentum mapping  conserve the invariant mass of this particle.
The condition \cref{eq:1initial:pR2} then enforces
\begin{equation}
	(\xi_a p_a + \xi_b p_b - p_A - p_B + p_R)^2
	= p_R^2.
\end{equation}
This is one quadratic equation in the two unknowns $\xi_a$ and $\xi_b$,
and is not sufficient to determine completely the mapping.
Changing variables to the product and the ratio of the momentum fractions
\begin{equation}
	\begin{cases}
		\displaystyle
		\xi \equiv \xi_a \xi_b,\phantom{\frac{\xi_a}{\xi_b}}\\
		\displaystyle
		t \equiv \frac{1}{2}\log\frac{\xi_a}{\xi_b},
	\end{cases}
	\qquad
	\begin{cases}
		\displaystyle
		\xi_a = \sqrt{\xi} e^{+t},\phantom{\frac{\xi_a}{\xi_b}}\\
		\displaystyle
		\xi_b = \sqrt{\xi} e^{-t},\phantom{\frac{\xi_a}{\xi_b}}
	\end{cases}
\end{equation}
we find the quadratic equation in $\sqrt{\xi}$
\begin{equation}
\label{eq:2initial:xiprod}
	(p_a + p_b)^2 \xi
	- 2 (e^{+t} p_a + e^{-t} p_b) \cdot (p_A + p_B - p_R) \sqrt{\xi}
	+ (p_A + p_B - p_R)^2 - p_R^2
	= 0.
\end{equation}

% Heuristic condition on the ratio
In order to be compatible with the one-sided initial-collinear mapping,%
\footnote{
See \cref{ssec:madnklo:NNLOdisjoint} for the final-state analogous
of this compatibility condition.
}
the transformation should reproduce \cref{eq:1initial:xia}
in the limit $p_B \to p_b$,
and a similar mechanism is required to work in the limit $p_A\to p_a$.
This means that the ratio between the momentum fractions
is supposed to reduce to
\begin{equation}
	\frac{\xi_a}{\xi_b} = \frac{(p_A-p_R)^2-p_R^2}{2p_a(p_A-p_R)},
\end{equation}
for $p_B \to p_b$, and
\begin{equation}
	\frac{\xi_a}{\xi_b} = \frac{2p_b(p_B-p_R)}{(p_B-p_R)^2-p_R^2},
\end{equation}
for $p_A \to p_a$.
Since both ratios on the \gls{RHS} reduce to one if the other limit
$p_A \to p_a$ ($p_B \to p_b$) is also taken,
as required to reproduce the starting phase-space point in the limit,
it is easy to see that taking their product
\begin{equation}
\label{eq:2initial:xiratio}
	\frac{\xi_a}{\xi_b} =
	\frac{2p_b(p_B-p_R)}{2p_a(p_A-p_R)}
	\frac{(p_A-p_R)^2-p_R^2}{(p_B-p_R)^2-p_R^2},
\end{equation}
satisfies the compatibility condition.
Starting from the full phase-space point,
it is thus possible to use this last equation to find $t$;
the coefficients of the quadratic equation for $\sqrt{\xi}$
are then all known and $\xi$ can be fixed.

% Simplifications
We observe that, when the recoil occurs against the whole final state,
\cref{eq:2initial:xiratio,eq:2initial:xiprod}
reduce to the simpler expressions
\begin{equation}
	\frac{\xi_a}{\xi_b} = \frac{(p_A+p_b)^2}{(p_a+p_B)^2},
	\qquad
	\xi_a \xi_b = \frac{p_R^2}{(p_a+p_b)^2}
	= \frac{(p_A+p_B)^2}{(p_a+p_b)^2}.
\end{equation}

% Lorentz boost
Once the transformation for a single recoiler is determined,
it is easy to generalise to an arbitrary number of recoilers
by first treating them collectively
and afterwards applying a Lorentz transformation to each of them.

